Space applications of GAGG:Ce scintillators: a study of afterglow emission by proton irradiation

We discuss the results of a proton irradiation campaign of a GAGG:Ce (Cerium-doped Gadolinium Aluminium Gallium Garnet) scintillation crystal, carried out in the framework of the HERMES-TP/SP (High Energy Rapid Modular Ensemble of Satellites -- Technological and Scientific Pathfinder) mission. A scintillator sample was irradiated with 70 MeV protons, at levels equivalent to those expected in equatorial and sun-synchronous low-Earth orbits over orbital periods spanning 6 months to 10 years. The data we acquired are used to introduce an original model of GAGG:Ce afterglow emission. Results from this model are applied to the HERMES-TP/SP scenario, aiming at an upper-bound estimate of the detector performance degradation resulting from afterglow emission.

==> sections/Afterglow/.trash/paramtable_old.tex <==
%
%
%\begin{table}[]
%\centering
%\resizebox{0.3\textwidth}{!}{%
%\begin{tabular}{llll}
%\toprule
%$n_i$ & $\sigma_n$ & $\tau_i$ & $\sigma_\tau$ \\
%\midrule
%$148.6$ & $2.8$ & $24.58$ & $0.42$ \\
%$66.8$ & $1.9$ & $68.04$ & $0.96$ \\
%$48.12$ & $0.40$ & $194.3$ & $1.7$ \\
%$20.32$ & $0.17$ & $697$ & $10$ \\
%$14.75$ & $0.16$ & $2213$  & $53$ \\
%$26.33$ & $0.18$ & $8.20 \cdot 10^3$ & $160$ \\
%$220.50$ & $0.80$ & $7.02 \cdot 10^4$ & $730$ \\
%
%\bottomrule
%\end{tabular}}
%\caption{params}
%\label{tab:finfit_nt}
%\end{table}
%
%
%\begin{table}[]
%\centering
%\resizebox{0.3\textwidth}{!}{%
%\begin{tabular}{llll}
%\toprule
%$\Phi$ & $\sigma_\Phi$ & $\Delta T_m$ & $\sigma_{\Delta T_m}$ \\
%\midrule
%$148.6$ & $2.8$ & $24.58$ & $0.42$ \\
%$66.8$ & $1.9$ & $68.04$ & $0.96$ \\
%$48.12$ & $0.40$ & $194.3$ & $1.7$ \\
%$20.32$ & $0.17$ & $697$ & $10$ \\
%$14.75$ & $0.16$ & $2213$  & $53$ \\
%$26.33$ & $0.18$ & $8.20 \cdot 10^3$ & $160$ \\
%$220.50$ & $0.80$ & $7.02 \cdot 10^4$ & $730$ \\
%
%\bottomrule
%\end{tabular}}
%\caption{params}
%\label{tab:finfit_phidelta}
%\end{table}



\begin{table}[]
\centering
    \begin{minipage}{.6\textwidth}
      \centering
       \resizebox{\textwidth}{!}{%
		\begin{tabular}{llllll}
		\toprule
		$\tau_i$ [$s$] & $\sigma_\tau$ [$s$] & $n_i$ [$cm^{-3}$]& $\sigma_n$ [$cm^{-3}$] & $\Delta n$ [$cm^{-3}$]& $\sigma_{\Delta n}$ [$cm^{-3}$]\\
		\midrule
		%$144.5$ & $53.1$ & $7.02 \cdot 10^4$ & $730 \\
		
		$24.7$ & $0.4$ & $205$ & $3$ & $73.0$ &  $3.8$\\
		$68.2$ & $0.9$ & $128$ & $1$ & $-15.0$ & $1.0$\\
		$191$ & $2$ & $100$ & $1$ & $-22.6$ & $0.7$\\
		$670$ & $10$ & $50.1$ & $0.8$ & $-22.6$ & $1.1$\\
		$2124$ & $48$ & $36.7$ & $0.7$ & $-16.8$ & $1.2$\\
		$8028$ & $148$ & $48.7$ & $0.3$ & N/A & N/A\\
		$6.910\cdot 10^4$ & $661$ & $408$ & $1$ & N/A & N/A\\


		\bottomrule
		\end{tabular}}
		\caption{Traps properties as estimated from fit to the model of Sec. \ref{sec:afterglow}. Afterglow data from a GAGG:Ce sample at temperature $21 \pm 0.5 \, ^\circ$C.}
		\label{tab:finfit_nt}
    \end{minipage}
\end{table}

==> sections/Afterglow/.trash/paramtable_older.tex <==
%
%
%\begin{table}[]
%\centering
%\resizebox{0.3\textwidth}{!}{%
%\begin{tabular}{llll}
%\toprule
%$n_i$ & $\sigma_n$ & $\tau_i$ & $\sigma_\tau$ \\
%\midrule
%$148.6$ & $2.8$ & $24.58$ & $0.42$ \\
%$66.8$ & $1.9$ & $68.04$ & $0.96$ \\
%$48.12$ & $0.40$ & $194.3$ & $1.7$ \\
%$20.32$ & $0.17$ & $697$ & $10$ \\
%$14.75$ & $0.16$ & $2213$  & $53$ \\
%$26.33$ & $0.18$ & $8.20 \cdot 10^3$ & $160$ \\
%$220.50$ & $0.80$ & $7.02 \cdot 10^4$ & $730$ \\
%
%\bottomrule
%\end{tabular}}
%\caption{params}
%\label{tab:finfit_nt}
%\end{table}
%
%
%\begin{table}[]
%\centering
%\resizebox{0.3\textwidth}{!}{%
%\begin{tabular}{llll}
%\toprule
%$\Phi$ & $\sigma_\Phi$ & $\Delta T_m$ & $\sigma_{\Delta T_m}$ \\
%\midrule
%$148.6$ & $2.8$ & $24.58$ & $0.42$ \\
%$66.8$ & $1.9$ & $68.04$ & $0.96$ \\
%$48.12$ & $0.40$ & $194.3$ & $1.7$ \\
%$20.32$ & $0.17$ & $697$ & $10$ \\
%$14.75$ & $0.16$ & $2213$  & $53$ \\
%$26.33$ & $0.18$ & $8.20 \cdot 10^3$ & $160$ \\
%$220.50$ & $0.80$ & $7.02 \cdot 10^4$ & $730$ \\
%
%\bottomrule
%\end{tabular}}
%\caption{params}
%\label{tab:finfit_phidelta}
%\end{table}



\begin{table}[]
    \begin{minipage}{.3\textwidth}
      \centering
       \resizebox{\textwidth}{!}{%
		\begin{tabular}{llll}
		\toprule
		$n_i$ [$cm^{-3}$]& $\sigma_n$ [$cm^{-3}$]& $\tau_i$ [$s$] & $\sigma_\tau$ [$s$] \\
		\midrule
		$97$ & $36$ & $24.58$ & $0.42$ \\
		$43$ & $16$ & $68.04$ & $0.96$ \\
		$31$ & $11$ & $194.3$ & $1.7$ \\
		$13.3$ & $4.9$ & $697$ & $10$ \\
		$9.6$ & $3.5$ & $2213$  & $53$ \\
		$17.2$ & $6.3$ & $8.20 \cdot 10^3$ & $160$ \\
		$144.5$ & $53.1$ & $7.02 \cdot 10^4$ & $730$ \\
		
		\bottomrule
		\end{tabular}}
		\caption{Traps characteristics as estimated from fit to the model of Sec. \ref{sec:afterglow}. Afterglow data from a GAGG:Ce sample at temperature $21 \pm 0.5 \, ^\circ$C.}
		\label{tab:finfit_nt}
    \end{minipage}
    \hfill
    \begin{minipage}{.55\textwidth}
      \centering
      \resizebox{\textwidth}{!}{%
		\begin{tabular}{lllll}
		\toprule
		$\Phi$ [$p\cdot cm^{-2} \cdot s^{-1}$]  & $\sigma_\Phi$  [$p\cdot cm^{-2} \cdot s^{-1}$] & $\Phi^M - \Phi$  [$p\cdot cm^{-2} \cdot s^{-1}$] & $\Delta T^m$ [$s$] & $\sigma_{\Delta T^m}$ [$s$] \\
		\midrule
		$1.524\cdot 10^6$ & $3.2\cdot 10^3$ & $-2.0\cdot 10^5$ & $20.48$ & $0.28$ \\
		$1.322\cdot 10^6$ & $3.3\cdot 10^3$ & $1.1\cdot 10^4$ & $9.16$ & $0.27$ \\
		$1.359\cdot 10^6$ & $3.1\cdot 10^3$ & $-4.0\cdot 10^4$ & $9.58$ & $0.52$ \\
		$1.37\cdot 10^7$ & $ 0.00 $ & $0.0$ & $9.754$ & $0.092$ \\
		$1.315\cdot 10^7$ & $1.3\cdot 10^4$ & $3.9\cdot 10^5$ & $8.573$  & $0.094$ \\
		$1.036\cdot 10^8$ & $7.6\cdot 10^4$ & $2.8\cdot 10^7$ & $0.00$ & $0.00$ \\
		
		\bottomrule
		\end{tabular}}
		\caption{Fluxes and delays as estimated from fit to the model outlined in Sec. \ref{sec:afterglow}. In the third column we list discrepancies between the best fit estimates and nominal value.}
		\label{tab:finfit_phidelta}
	\end{minipage}
\end{table}

==> sections/Afterglow/afterglow.tex <==
\section{Afterglow emission and decrease in light-yield resulting from irradiation with protons}
\label{sec:afterglow}

Long-lived afterglow emission in scintillators is attributed to the existence of intrinsic or impurity defects within the crystal lattice. Some of the charge carriers (electrons or holes) liberated by the ionizing radiation can be trapped at defect sites into metastable states. At later times, charge carriers can escape these sites by different processes (e.g. to the conduction band by thermal energy absorption \cite{knoll} or to nearby reconbination centers by direct or thermally assisted tunneling \cite{2006:huntley}). Ultimately all of the charge carriers recombine, mainly through radiative paths in good scintillators, giving rise to luminescence.  Different scintillators display different afterglow characteristics, varying from almost non-existent to a very long and intense emission \cite{Yoneyama_2018}. Although mitigation techniques, such as Mg-codoping, proved successful \cite{LUCCHINI2016176}, GAGG:Ce has been known to belong to the end of the spectrum showing intense emission lasting up to several days \cite{Yoneyama_2018}.\\
In the existing literature GAGG:Ce afterglow emission has been reported decaying as a power-law of time with power index near $- 1.0$. Such a model would be compatible with afterglow emission resulting from tunnelling of trapped electrons to randomly distributed recombination centres \cite{LUCCHINI2016176} \cite{2006:huntley}. We find this description  troublesome. If on one hand we find power-laws able to reproduce luminescence lasting between $10^2$ and $10^3$ s with good accuracy, on the other they fail to describe emissions sustained for times greater than about $10^3$ s, as evident from Fig. \ref{fig:allrun}.
This behaviour was observed both for luminescence resulting from scintillator samples irradiated with protons and exposed to daylight.
Moreover, even in the time interval between tens and hundreds of seconds, residual analysis from power-law fit show systematic patterns which proved difficult to justify, see Fig. \ref{fig:powlawresidual}.
We do not exclude tunnelling effects to play a role in afterglow emission. However we find such a model to be unable to fully explain our observations.
We add that, being unable to capture the nuances of sustained emission, power-law models are particularly problematic for the purpose of this work. In fact, failing at larger time-scales, they may result in an inaccurate description of accumulation effects which we expect as a result of the continuos irradiation taking place in orbit.\\
\begin{figure}
\centering
\includegraphics[width=0.7\textwidth]{img/firstrun-powlaw}
\caption{Fit to inverse power-law plus a background constant of curve '2019.01.30 19:59', cf. Tab. \ref{tab:FULLdoses}. Best fit power-law index is $1.54$. Time-dependent patterns in residuals are apparent.}
\label{fig:powlawresidual}
\end{figure}
%2. Even in the time interval between tens and hundreds of seconds, residual analysis from power-law fit shows a systematic pattern which proves difficult to justify. In Fig. \ref{fig:powlawresidual} a typical fit to power-law plus background constant of a GAGG:Ce afterglow decay curve is shown along with the residuals. 
%3. As will be clear in the following, we need a model of afterglow which should be flexible enough to deal with a range of irradiation durations and fluxes i.e., a semi-analytical model of sort. 
%Analytically dealing with power-law is impractical.
%\begin{figure}
%\centering
%\includegraphics[width=0.7\textwidth]{img/longrun}
%\caption{PMT anode current resulting from afterglow emission of a GAGG:Ce scintillator sample, stimulated through $5$ minutes exposure to daylight. The observed afterglow luminescence differs from index $\sim -1$ power-laws already few hundreds of seconds after the illumination ended.}
%\label{fig:longrun}
%\end{figure}


All the above considered, we propose a simple semi-empirical model based on the idea that afterglow emission could result from the presence of traps with few different, discrete energetic levels from which charge carriers can escape through thermal excitation.\\
Our measurements are not able to identify the charge carriers involved in these processes, whether they are electrons or holes, so we should continue to speak about charge carriers. However, to simplify the discussion, in the following we refer only to trapping of electrons. The same reasoning applies also to the holes. \\
We make a number of simplifying assumptions motivated by the fact that our observations are largely unable to account for the details of the physical processes at play.
\begin{enumerate}
\item We assume irradiation with protons to occur with constant flux for the entire duration of each irradiation step. Moreover, the proton beam is considered uniformly distributed on the entire crystal. This approximation, although useful, is inaccurate. In fact, as mentioned in Sec. \ref{sec:expout}, the TPTC proton beam extraction current is modulated by a 50\% duty-cycle square wave with a 100 ms period \cite{TPTC}. This period is small when compared to the time elapsed between the end of the irradiations and the start of the measurements ($60$ s). Hence we expect the beam's intensity square modulation to have little impact on the quality of the model's prediction.
\item We consider traps to be uniformly distributed in the crystal volume.
\item We neglect fluctuations in the ionization, by using averages, and the details of the electron capture processes. We assume the time spent by an electron in the conduction band to be very small in comparison with the timescales of the other processes.
\item At the same time we assume that electrons will always encounter traps of every type. This implies that the probability for an electron to get trapped does not depend on the number of traps already occupied hence excluding possible saturations effects from our model.
\item Finally, we assume that electrons escaping from a trap are not trapped again. (NZ)
 \end{enumerate}
Since we assumed that the probability for an electron to get trapped does not depend on the number of traps already occupied and the number of particles (protons or photons, exited electrons) involved in the relevant processes during an irradiation step is large, we can assume that the number of electrons $N_i$ captured by a particular $i$-labelled trap species varies with time through the differential law:
The fourth simplifying assumption allows for an independent treatment of electron capture by the different trap species, so for the number of electrons $N_i$ captured by a particular $i$-labelled trap species we can write the following differential equation:
\begin{equation}
\frac{dN_i}{dt} = n_i \Phi - \frac{N_i}{\tau_i}
\end{equation}
The first term on the RHS accounts for electrons trapped during irradiation. Hence, $\Phi$ is the radiation flux integrated on the crystal volume, $n_i$ is the average number of electrons trapped for particle of incident radiation and $\tau_i$ is the average lifetime of this particular metastable state. For simplicity we will often refer to the former parameter as the 'traps numbers'.\\
The second term accounts for the electron emission from the traps, which happens with a rate that is proportional to the reciprocal of their mean lifetime in this particular metastable state.\\
The general solution to the equation above is:
\begin{equation}
N_i(t) = N_{i,0} e^{-\frac{t}{\tau_i}} + n_i \Phi \tau_i (1 - e^{-\frac{t}{\tau_i}})
\end{equation}
where $N_{i,0}$ indicates the traps already occupied %before irradiation starts. (NZ)
at the start time of the irradiation.
If the irradiation has finite duration $\Delta t_I$, the number of trapped electrons at a time $t$ from the end of irradiation is:
\begin{equation}
N_i(t) = [
N_{i,0} e^{-\frac{\Delta t_I}{\tau_i}} + 
n_i \Phi \tau_i (1 - e^{-\frac{\Delta t_I}{\tau_i}})
] 
e^{-\frac{t}{\tau_i}} 
\label{eq:trapag}
\end{equation}
The resulting current $I(t)$ measured from the picoammeter would correspond to:
\begin{equation}
I(t) = - e f \epsilon_V G_V \frac{dN}{dt}
\label{eq:current}
\end{equation}
Where $e$ is the elementary charge, $f$ the photon transport efficiency from crystal to the photocathode, $\epsilon_V$ the quantum efficiency of the PMT and $G_V$ its gain at operational voltage $V$.\\
We will employ the value $G_{1500} = (1.04 \pm 0.04)\cdot 10^6$ as justified in \ref{sec:calibration}. The PMT quantum efficiency strongly depends on the incident light spectrum. 
Interpolating the GAGG:Ce afterglow emission spectrum with the PMT spectral quantum efficiency, as reported in \cite{Yoneyama_2018} and \cite{hamamatsu_tubes}, we recover  $\epsilon_V = 0.06 \pm 0.01$.
Another quantity depending on the incident wavelength is the photon transport efficiency from crystal to the photocathode, $f$. We will adopt a value $f = 0.61 \pm 0.18$.
We motivate the choice of this value stating that observations of the emission following the absorption of $662$ keV photons from a Cs-137 source resulted in a best estimate of the effective light output of $31 \pm 9$ photons/keV for the ‘J2’ GAGG:Ce, post-irradiation, teflon-wrapped sample, coupled by means of silicone grease to a pair of photomultiplier as in Fig. \ref{fig:expsetup}.
Our estimate of photon transport efficiency from crystal to photocathode $f$ was obtained by dividing the measured effective light output by the sample manufacturer nominal light output measurement $53 \pm 3$ photon/keV \cite{gaggJ2}. \\
We observed a small degradation in light-output resulting from proton irradiation of GAGG:Ce up to a dose value roughly equivalent to that expected from $10$ years of sun-synchronous orbit.
Data are reported in Tab. \ref{tab:outputdegradation_J1} and Fig. \ref{fig:outputdegfig} implying a moderate light-yield reduction of $3.7 \pm 1.2 \%$. This effect was taken into account in our estimate of the photon transport efficiency.
\begin{figure}[h!]
\centering
\includegraphics[width = 0.7\textwidth]{img/outputdegradation}
 	\caption{Maximum amplitude histogram from 70 MeV protons scintillation event, before (blue) and after (orange)  irradiation with $(2.95 + 0.05) \cdot 10^{10}$ protons. Only small variations in peak position were observed, accounting for reduction in light-yield of $3.7 \pm 1.2 \%$.}
	\label{fig:outputdegfig}
\end{figure}
\input{./sections/RadTolerance/lyieldtable}

Given that a reduction in scintillator light-yield following proton irradiation was indeed observed, it makes sense to extend our starting model to support a dose-dependent variation in the afterglow emission too.
In our model framework, such variations can be described accounting for  creation or annihilation of the traps available to a single specie or correlation effects between different species.  
It is not possible to identify the exact physical mechanisms responsible for such phenomena within the available data. 
We should therefore proceed in an approximate way. We relax hypothesis 4 and for semplicity sake assume the traps numbers $n_i$ to changes linearly with the irradiation dose, a simplification which we expect to give good results if the variation in afterglow emission is small. 
The number of electrons trapped during the irradiation step $j$ is determined by the equation:
\begin{equation}
\label{eq:new_mod_eq}
 \frac{d N_i}{dt} = n_{i,j} \phi_j - \frac{N_i}{\tau_i}
\end{equation}
where we assume that $n_{i,j}$ change linearly with the accumulated dose:
$$ n_{i,j} (t) = n_{i,j-1} + k_i \phi_j t $$ 
and note $n_{i,j-1}$ the $i$-species trap number at the end of the $j-1$ irradiation step.\\
In turns, $n_{i,j-1}$ will depend from the irradiation dose of the $j-2$ step and so forth. Going back to the first irradiation we can write:
$$   n_{i,j-1} = n_{i0} + k_i\sum_{l=1}^{j-1}\phi_l T_l $$
The general solution to Eq. \ref{eq:new_mod_eq} is:
$$   N_i(t) = N_{i,j0}e^{-t/\tau_i}+n_{i,j-1}\tau_i\phi_j(1-e^{-t/\tau_i})+k_i\tau_i^2\phi_j^2 [t/\tau_i-(1-e^{-t/\tau_i})]$$
Once the irradiation ceases the number of electrons occupying the $i$-traps decrease exponentially with time, $\propto e^{-t/ \tau_i}$. The measured current will be proportional to the time derivative of $N_i$, in the same way we outlined for the first model, hence:
$$ I_i(t) \propto [(n_{i,j-1}-k_i\tau_i\phi_j)\phi_j(1-e^{-T_j/\tau_i})+k_i T_j\phi_j^2]e^{-t/\tau_i} $$
In the following we will always express the variation in trap number through the total variation observed at the end of the last irradiation, $\Delta  n_i = k_i \sum_j \phi_j T_j = k_i \Phi_{TOT}$. According to this definition, the variation in trap number predicted by the model for an intermediate fluence $\Phi$ will be expressed by:
\begin{equation}
\label{eq:scaled_ns}
\Delta  n_i \frac{\Phi}{\Phi_{TOT}}
\end{equation}


In fitting our observation to the model, we begin associating uncertainties to the dataset. Uncertainties are computed as residuals of a cubic-spline fit of the irradiation lightcurves.
Fig. \ref{fig:rms} shows the computed RMS values along the different components of the dataset. We found a reasonable empirical parametrization of the RMS curves in $ RMS = A+B\cdot I^C$. Best fit to this law is shown as a solid black line.
\begin{figure}[h!]
\centering
\includegraphics[width=0.7\textwidth]{img/rms}
\caption{RMS values computed from residuals to cubic-spline fit. The set in red behaving differently represent nightly afterglow monitors following highest dose irradiation. Since the fluctuations seem to be smaller than the trend we neglect this dataset and model RMS as $RMS = A+B\cdot I^C$. Best fit to this law is shown in black solid line and refers to values: $A = 0$, $B = 0.35$ and $C = 0.49$. See Tab. \ref{tab:FULLdoses} for color legend.}
\label{fig:rms}
\end{figure}
The fitting routines initialize considering only the data from the first few irradiation steps, then progressively add subsequent measurements. At each iteration the partial model is used to assess the robustness of the prediction for the following irradiations and to determine which adjustments are needed to successfully fit the whole dataset.\\
We must now remark on a crucial weakness of our observations. All the informations about proton-induced afterglow emission at large time scales come from a single observation, the last one, which was protracted during the night following the irradiations. For this reason, it is presently not possible to adequately constrain eventual variations in the parameters characterizing the traps with average lifetime much longer than $800$~s. For this reason we choose to avoid taking into account dose-dependent variations in trap numbers for these components.

\begin{figure}[h!]
\centering
\includegraphics[width=0.8\textwidth]{img/finfit}
\caption{Best fit of the January 30th dataset to the model of Sec. \ref{sec:afterglow}. Parameters estimates are reported in Tab. \ref{tab:finfit_nt}. Temperatures in range $21 \pm 0.5 \, ^\circ$C} 
\label{fig:finfit}
\end{figure}
\input{./sections/Afterglow/paramtable}
Fit results are graphically reported in Fig. \ref{fig:finfit}, while the best fit parameters values are reported in Tab. \ref{tab:finfit_nt}. We find seven to be the smallest number of trap species needed to resolve patterns in fit residuals. Employing more trap species results in worse estimates of best fit parameters and no significant improvements in the residuals.\\

==> sections/Afterglow/afterglow_old.tex <==
\section{Afterglow emission resulting from irradiation with protons}
\label{sec:afterglow}

Long-lived afterglow emission in scintillators is attributed to the existence of intrinsic or impurity defects within the crystal lattice. Some of the electrons promoted to the conduction band by the ionizing radiation can be trapped at defect sites into metastable states. At later times, trapped electrons can escape these sites by different processes (e.g. to the conduction band by thermal energy absorption \cite{knoll} or to nearby reconbination centers by direct or thermally assisted tunneling \cite{2006:huntley}). Ultimately all of the electrons recombine, mainly through radiative paths in good scintillators, giving rise to luminescence.  Different scintillators displays different afterglow characteristics, varying from almost non-existent to a very long and intense emission \cite{Yoneyama_2018}. Although mitigation techniques, such as Mg-codoping, proved successful \cite{LUCCHINI2016176}, GAGG:Ce has been known to belong to the end of the spectrum showing intense emission lasting up to several days \cite{Yoneyama_2018}.\\
In the existing literature GAGG:Ce afterglow emission has been reported decaying as a power-law of time with power index near $- 1.0$  \cite{LUCCHINI2016176} \cite{Yoneyama_2018}. This description is troublesome for the following reasons.
1. Afterglow time signatures fail to approximate a power-law for times greater than $10^3$ s or less.
PMT anode current resulting from afterglow emission of a GAGG:Ce scintillator sample, stimulated through $5$ minutes exposure to daylight. The observed afterglow luminescence differs from index $\sim -1$ power-laws already few hundreds of seconds after the illumination ended., cf Fig. \ref{fig:longrun}. 
This is problematic since failing to describe afterglow on long time-scales will result in an inaccurate description of accumulation effects we expect to take place in orbit.
2. Even in the time interval between tens and hundreds of seconds residual analysis from power-law fit shows a pattern which proves difficult to justify. In Fig. \ref{fig:powlawresidual} a typical fit to power-law plus background constant of a GAGG:Ce afterglow decay curve is shown along with the residuals. 
3. As will be clear in the following, we need a model of afterglow which should be flexible enough to deal with a range of irradiation durations and fluxes i.e., a semi-analytical model of sort. Analytically dealing with power-law is impractical.
\begin{figure}
\centering
\includegraphics[width=0.7\textwidth]{img/longrun}
\caption{PMT anode current resulting from afterglow emission of a GAGG:Ce scintillator sample, stimulated through $5$ minutes exposure to daylight. The observed afterglow luminescence differs from index $\sim -1$ power-laws already few hundreds of seconds after the illumination ended.}
\label{fig:longrun}
\end{figure}
\begin{figure}
\centering
\includegraphics[width=0.7\textwidth]{img/firstrun-powlaw}
\caption{Fit to inverse power-law plus a background constant of curve '2019.01.30 19:59', cf. Tab. \ref{tab:FULLdoses}. Best fit power-law index is $-1.044$. Time-dependent patterns in residuals are apparent.}
\label{fig:powlawresidual}
\end{figure}\\

All the above considered, we propose a simple semi-empirical model based on the idea that afterglow emission could result from the presence of traps with different, discrete energetic levels from which electrons can escape through thermal excitation.\\
We make a number of assumptions motivated by the fact that our observations are largely unable to account for the details of the physical processes at play.
\begin{enumerate}
\item We assume irradiation with protons to occur with constant flux for the entire duration of each irradiation step. Moreover, the proton beam is considered uniformly distributed on the entire crystal. This approximation, although useful, is unaccurate. In fact, as mentioned in Sec. \ref{sec:expout}, the TPTC proton beam extraction current is modulated by a 50\% duty-cycle square wave with a 100 ms period \cite{TPTC}. 
\item We consider traps to be uniformly distributed in the crystal volume. 
\item We neglect fluctuations in the ionization, by using averages, and the details of the electron capture processes. We assume the time spent by an electron in the conduction band to be very small in comparison with the timescales of the other processes.
\item At the same time we assume that electrons will always encounter traps of every type. This implies that the probability for an electron to get trapped does not depend on the number of traps already occupied hence excluding possible saturations effects from our model.
\item Finally, we assume that electrons escaping from a trap are not trapped again.
 \end{enumerate}
Since we assumed that the probability for an electron to get trapped does not depend on the number of traps already occupied and the number of particles (protons or photons, exited electrons) involved in the relevant processes during an irradiation step is large, we can assume that the number of electrons $N_i$ captured by a particular $i$-labelled trap species varies with time through the differential law:
\begin{equation}
\frac{dN_i}{dt} = n_i \Phi - \frac{N_i}{\tau_i}
\end{equation}
The first term on the RHS accounts for electrons trapped during irradiation. Hence, $\Phi$ is the radiation flux integrated on the crystal volume, $n_i$ is the average number of electrons trapped for particle of incident radiation and $\tau_i$ is the average lifetime of this particular metastable state.\\
The general solution to the equation above is:
\begin{equation}
N_i(t) = N_{i,0} e^{-\frac{t}{\tau_i}} + n_i \Phi \tau_i (1 - e^{-\frac{t}{\tau_i}})
\end{equation}
where $N_{i,0}$ indicates the traps already occupied before irradiation starts. 
If the irradiation has finite duration $\Delta t_I$, the number of trapped electrons at a time $t$ from the end of irradiation is:
\begin{equation}
N_i(t) = [
N_{i,0} e^{-\frac{\Delta t_I}{\tau_i}} + 
n_i \Phi \tau_i (1 - e^{-\frac{\Delta t_I}{\tau_i}})
] 
e^{-\frac{t}{\tau_i}} 
\label{eq:trapag}
\end{equation}
The resulting current $I(t)$ measured from the picoammeter would correspond to:
\begin{equation}
I(t) = - e f \epsilon_V G_V \frac{dN}{dt}
\label{eq:current}
\end{equation}
Where $e$ is the elementary charge, $f$ the photon transport efficiency from crystal to the photocathode, $\epsilon_V$ the quantum efficiency of the PMT and $G_V$ its gain at operational voltage $V$.\\
We will employ the value $G_{1500} = (1.04 \pm 0.04)\cdot 10^6$ as justified in Sec. \ref{sec:calibration}. The PMT quantum efficiency strongly depends on the incident light spectrum. Making the simplifying assumption that the GAGG:Ce afterglow light is monochromatic at $520$ nm (the crystal emission peaks at this wavelength, cf. \cite{Yoneyama_2018}) we assume  $\epsilon_V = 0.1 \pm 0.01$, from \cite{hamamatsu_tubes}.
Another quantity depending on the incident wavelength is the photon transport efficiency from crystal to the photocathode, $f$. We will adopt a value $f = 0.61 \pm 0.18$.
We motivate the choice of this value stating that observations of the emission following the absorption of $662$ keV photons from a Cs-137 source resulted in a best estimate of the effective light output of $31 \pm 9$ photons/keV for the 'J2' GAGG:Ce, post-irradiation, teflon-wrapped sample, coupled by means of silicone grease to a pair of photomultiplier as in Fig. \ref{fig:expsetup}.
Our estimate of photon transport efficiency from crystal to photocathode $f$ was obtained by dividing the measured effective light output by the sample manufacturer nominal light output measurement $53 \pm 3$ photon/keV \cite{gaggJ2}, taking into account a light yield degradation of $3.7 \pm 1.2 \%$ (see Sec. \ref{sec:radtol}). 
%Within the error range, values of effective and nominal light-output were chosen in such a way to provide an upper-bound estimate of afterglow luminescence---compatibly to the approach of Sec. \ref{sec:leakage}. \\

The model outlined above is now applied to the data acquired during January 30th. Unless stated otherwise, we will refer to this subset of data as our dataset.  
Through a fitting procedure we will attempt to derive the model parameters i.e., $\tau_i$, trap emission time constants, and $n_i$, average number of electrons trapped for particle of incident radiation. 
We will also treat as free parameters some of the variables which were affected by uncertainties during the measurements, namely the flux values, the time elapsed between the end of an irradiation and the start of the measurement, and---unless stated otherwise---the dark current of the PMT.\\
The objective function used for the calculation of the fit residuals is outlined in Listing \ref{lst:obj_fun}. Parameters for fluxes and irradiation durations were intialized and constrained according to the values reported in Tab. \ref{tab:FULLdoses}. We note that flux values were estimated from a GEANT4 simulation of the number of beam protons intercepted by the scintillator sample.
\input{./sections/Afterglow/obj_function}
We begin our analysis evaluating the uncertainties in data from the residuals of a cubic-spline fit of the irradiation lightcurves.
Fig. \ref{fig:rms} shows the RMS values computed from spline-fit residuals along the different components of the dataset. We found a reasonable empirical parametrization of the RMS curves in $ RMS = A+B\cdot\sqrt I+C\cdot I$. Best fit to this law is shown as a solid black line.
\begin{figure}[h!]
\centering
\includegraphics[width=0.7\textwidth]{img/rms}
\caption{RMS values computed from residuals to cubic-spline fit. The set in red behaving differently represent nightly afterglow monitors following highest dose irradiation. Since the fluctuations seem to be smaller than the trend we neglect this dataset and model RMS as $ RMS = A+B\cdot\sqrt I+C\cdot I$. Best fit to this law is shown in black solid line. Cf. Tab. \ref{tab:FULLdoses} for color legend.}
\label{fig:rms}
\end{figure}
At this point we can assign an uncertainty value to current measurements in the dataset and begin to fit the model to the dataset.\\ 
\begin{figure}[ht!] 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth]{img/5Five} 
    \caption{Five different trap species.} 
    \label{fig7:a} 
    \vspace{4ex}
  \end{subfigure}%% 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth]{img/6Six} 
    \caption{Six different trap species.} 
    \label{fig7:b} 
    \vspace{4ex}
  \end{subfigure} 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth]{img/7Seven} 
    \caption{Seven different trap species.} 
    \label{fig7:c} 
  \end{subfigure}%%
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth]{img/8Eight} 
    \caption{Eight different trap species.} 
    \label{fig7:d}    
  \end{subfigure} 
  \caption{Residuals corresponding fit to models with different number of trap species for afterglow emission resulting from last irradiation run of day January 30th. While five and six different trap species are not enough to fully resolve patterns in residuals, eight species results in no significant improvements. for the sake of clarity only the first $\sim 20000$ s are shown. See Fig. \ref{fig:seventraps} for an example of fit over an entire acquisition.}
  \label{fig:trapspecies} 
\end{figure}
\begin{figure}[h!]
\centering
\includegraphics[width=0.7\textwidth]{img/seventraps}
\caption{Fit to a model with seven traps species of acquisition '2019.01.30 22:02' (sixth run of January 30th).}
\label{fig:seventraps}
\end{figure}
In order to assess the number of trap species we focus on the data from the last irradiation of the day. We find seven to be the smallest number of trap species needed to resolve patterns in fit residuals. Employing more trap species results in worse estimates of best fit parameters and no significant improvements in residuals, cf. Fig. \ref{fig:trapspecies} and Fig. \ref{fig:seventraps}.\\
\begin{figure}[h!]
\centering
\includegraphics[width=0.6\textwidth]{img/baseline}
\caption{Residuals from fit to seven-traps model of the last measurements run of January 30th for different values of anode baseline current $I_b$ spanning range  $79$--$84$ nA with $0.5$ nA resolution. Procedure was repeated for parameters initialized at very different values with no significant discrepancies in results.}
\label{fig:baseline}
\end{figure}
During measurements we had no means to reliably quantify $I_b$, the PMT dark current. This lack of information results in worse uncertainties for the parameters characterizing traps with the longest lifetimes. However, we can obtain a good approximation of $I_b$ by comparing residuals from several fits in which this parameter is fixed to different values. Results from a scan between $I_b$ values $79$ nA and $84$ nA with $0.5$ nA resolution is shown in Fig. \ref{fig:baseline}.
We report a best estimate of $I_b = 81.5293 \pm 0.0008$ nA. From now on we will cease to treat $I_b$ as a parameter and fix the phototube background constant in our model to this value. \\
One of the problems we face in this work concerns the uncertainties in proton fluxes. In theory, we can express proton fluxes as free fit parameters. However, since the $j-$th fluxes $\Phi_j$ multiply the trap parameters $n_i$, the model is invariant under scaling of all the fluxes by a parameter $k_1$ if simultaneously the $n_i$ are rescaled by a factor $1/k_1$. 
This ambiguity impacts our best estimate of the error on the $n_i$ parameters.
We consider the best estimate of the $j-$th run beam flux obtained from the fit to our model $\Phi_j^M = k_1 \Phi_j$. Weighting the fluxes \footnote{We remark that since irradiation fluxes spanned different orders of magnitude it was necessary to weight the nominal and model fluxes opportunely. 
We choose the beam intensity as our weights. A different choice of the weights (e.g. nominal fluxes values or uncertainty) is equally possible: results would sligthly differ without the outcome changing. } we find that the model estimate $\Phi_j^M$ closest to the nominal value $ \Phi_j$ is achieved for the fourth run of the dataset ($j = 4 $, '2019.01.30 21:12 ', as in Tab. \ref{tab:FULLdoses}).
This implies that $\Phi_4^M \sim \Phi_4$. Since we cannot improve the precision and accuracy of our flux measurements, we assume that in fact $\Phi_4^M = \Phi_4$ from which $k_1 = 1$, to which we associate an uncertainty $\Delta k_1 = \frac{ \Delta \Phi_4}{\Phi_4}$\\
A second problem concerns the uncertainties on the time intervals elapsed between the end of irradiations and the start of measurements.
Similiarly to what we have seen for $k_1$, uncertainties on the time delays elapsed between the end of irradiations and the start of measurements compromise our best estimates of $n_i$ parameters. In fact, the model is again invariant under summation of a constant $k_2$ to all the delays, if the parameters $n_i$ are simultaneously scaled by a factor $e^{+\frac{k_2}{\tau_i}}$. 
Noting with $T_j^M$ our model estimate of the delays elapsed between an irradiation end and the start of the acquisition, we have that $T_j^M = 60 s + \Delta T_j + k_2$. 
From the fit results we find $\Delta T_6$ to be the smallest estimated delay. For convenience we choose $k_2 = 0$, as it would be if $\Delta T_6 = 0$.\\ Associating an uncertainty to $k_2$ is not straightforward. 
In fact, this value will depend on the uncertainty $\Delta T_6$ which in turn  stems from the inherent unaccuracy of the manual procedure employed at the start of each measurement: beam control room communicated the end of an irradiation via phone and display device, a chronometer was started and after $60$ seconds the acquisition was started on the computer. In the following we will assume $\Delta k_2 = 1 s$.\\
Since $n_i = n_i^M e^{\frac{k_2}{\tau_i}}/k_1$, the values $k_1 = 1$ and $k_2 = 0$ will not impact the best model estimate of the $n_i$ parameters. However, the values of $\Delta n_i$ will be affected by the $k$ parameters and their uncertainties.\\
Neglecting the $I_b$ parameter--- the uncertainty of which is expected to have small impact on the final results---, the ambiguity of our model is all comprised in the parameters $k_1$ and $k_2$. We note that the considerations above have no impact on the fit estimates of the average trap lifetimes $\tau_i$.\\


Keeping in mind all the above we can finally fit our dataset. Results are presented in graphical form in Fig. \ref{fig:finfit} and in Tab. \ref{tab:finfit_nt} and \ref{tab:finfit_phidelta}.
Even if the model satisfingly reproduces the data, there are discrepancies between nominal values and fit estimates which could not be resolved in the present framework and could be due to excessive simplifications in our model.  In particular, it is likely that at highest doses radiation damage affected the number of available traps or was responsible for the formation of new trap species with different lifetimes.
None of the assumption we made are contradicted by data. 
In particular, the best values recovered for the $n_i$---as expressed in \ref{tab:finfit_nt}---are compatible with the assumption that the probability for an electron emitted from a metastable state to be trapped again is small. This is true since the ratio between the average number of trapped electrons per particle of incident radiation, $n_i$, and the average number of electrons which are brought in conduction band from a $70$ MeV proton is small, considering the average energy $\sim 15$ eV needed to create an electron-hole pair (as can be inferred from \cite{2018:kozlova} and \cite{2014:yanagida}).
\input{./sections/Afterglow/paramtable}
\begin{figure}[h!]
\centering
\includegraphics[width=\textwidth]{img/finfit}
\caption{Best fit of the January 30th dataset to the model of Sec. \ref{sec:afterglow}. Parameters estimates are reported in Tab. \ref{tab:finfit_nt} and \ref{tab:finfit_phidelta}. Temperatures in range $21 \pm 0.5 \, ^\circ$C} 
\label{fig:finfit}
\end{figure}


==> sections/Afterglow/lyieldtable.tex <==
%\begin{table}[]
%\centering
%\resizebox{\textwidth}{!}{%
%\begin{tabular}{l|c|c|c|}
%\cline{2-4}
% & \multicolumn{1}{l|}{Peak Position [channels]} & \multicolumn{1}{l|}{Energy Resolution [\%]} & Received Dose [protons] \\ \hline
%\multicolumn{1}{|l|}{Before Irradiation} & $2324 \pm 19$ & $25.1 \pm 2.2$ & - \\ \hline
%\multicolumn{1}{|l|}{After Irradiation} & $2237 \pm 19$ & $27.6 \pm 2.3$ & $(2.95 + 0.05) \cdot 10^{10}$ \\ \hline
%\end{tabular}%
%}
%\caption{Peak positions and energy resolution before and after proton irradiation.}
%\label{tab:outputdegradation}
%\end{table}
\begin{table}[hb!]
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{llll}
\toprule
 &Peak Position [channels] & FWHM Energy Resolution [\%] & Dose [protons]  \\
\midrule
Before Irradiation & $2324 \pm 19$ & $25.1 \pm 2.2$ & - \\
After Irradiation & $2237 \pm 19$ & $27.6 \pm 2.2$ & $(2.95 + 0.05) \cdot 10^{10}$ \\
\bottomrule
\end{tabular}}
\caption{Peak positions and energy resolution before and after proton irradiation corresponding to an observed light-yield reduction of $3.7 \pm 1.2 \%$.}
\label{tab:outputdegradation_J1}
\end{table}


==> sections/Afterglow/obj_function.tex <==
\begin{lstlisting}[language=Python,caption={The objective function used for the calculation of the fit residuals in pythonic pseudo-code. The dictionary \lstinline{v} contains the initialized fit parameters.},label={lst:obj_fun}]
def residual(pars, t, scaling, runs_to_fit, measured_values):
    from scipy.constants import elementary_charge as ECHARGE
    GAIN = 1.04 * 10 ** 6  
    PMT_EFF = 0.1 
    F = 0.61
    CORR_FAC = GAIN * PMT_EFF * F * ECHARGE* scaling
    DELAY = 60.0            # seconds

    v = pars.valuesdict()   # unpacking parameters

    model = v['Ib']
    for run_index, run in enumerate(runs_to_fit):
        for i in range(v['trap_number']):
            model += heaviside(t - (run.time_since_start - DELAY - v['dT_' + str(run_index)]), 1)* CORR_FAC * v['fluxN_' + str(run_index)] * (1 - run.irr_duration / v['exp_t' + str(i)])) * exp(-(t - (run.time_since_start - DELAY - v['dT_' + str(run_index)])) / v['exp_t' + str(i)])

    return model - measured_values
\end{lstlisting}

==> sections/Calibration/calibration.tex <==
\section{Instrument Calibration}
\label{sec:calibration}

At TPTC we worked with PMTs which are very different detectors with respect to SDDs, the detector technology chosen for HERMES. In fact PMT detectors are high-gain, low quantum efficiency devices while SDDs are characterized by no intrinsic gain and very high quantum efficiency. This implies that the scintillator afterglow emission has different consequences for the two systems. \\
On average, the afterglow emission appears to be a continuous stream of optical photons with a monotonically decreasing flux after stimulation. 
The randomly arriving photons are able to induce a detectable PMT anode current pulse, something that will not happen with the highly efficient but unamplifying SDDs. It follows that scintillator afterglow will not result in triggering the SDD front-end electronics, instead it will behave as an equivalent increase of the detector leakage current.\\
In order to translate our results with PMTs into effects on the SDDs we calibrated the PMT detectors employed at TPTC. We refer to the integral of the digitized waveform of the anode current pulses as the signal amplitude (in units of ADU $\cdot$ s).
We approached calibration as follows:
\begin{enumerate}
    \item \textit{PMT calibration.} We estimate $k_V$, the amplitude, at different supply voltages $V$, of the signal that would be produced by the extraction of a single photoelectron at the photocathode. To do so we employed a $400$ nm pulsed laser attenuated by filters of different opacity. Measurements were repeated for voltage values spanning $1000$--$1600$ V and the resulting waveforms digitized and recorded.
    \item \textit{Digitizer calibration.} We estimate $c$, the ratio between the anode pulse charge reaching the digitizer and the amplitude of the corresponding signal.
    \item \textit{Gain-voltage curve.} The voltage-gain curve is built and fitted according to the equation $G_V = c \cdot k_{V}/e$, where $e$ is the elementary charge.
\end{enumerate}

\paragraph{Phototube calibration}
%What amplitude would have a signal produced by an electron extracted from the PMT cathode?
We need to estimate the amplitude produced when a single electron is extracted from the PMT cathode.
For an average signal of amplitude $\mu$ we have that $\mu = k N_{pe}$ where $N_{pe}$ is the number of photoelectrons extracted at the cathode and $k$ is a proportionality constant expressed in ADU$\cdot $s$/$photoelectrons.
For a particular signal distribution, corresponding to a particular signal intensity, the expected signal variance can be expressed as:
\begin{equation}\label{eq:calibration}
\sigma^2 = \sigma^2_{noise} + \sigma^2_ {pois} + \sigma^2_{mult}
\end{equation}
where $\sigma^2_{noise}$ accounts for the electronic noise, $\sigma^2_{pois} = (k \sqrt{N_{pe}})^2$ is determined by the poissonian distribution of photoelectrons generated at the photocathode, while $\sigma^2_{mult} = \alpha (k N_{pe})^2$ describe the fluctuations intrinsic to the photomultiplication process.
Putting things together we have:

\begin{equation}\label{eq:calibration2}
\sigma^2 = \sigma^2_{noise} +(k \sqrt{N_{pe}})^2 + \alpha (k N_{pe})^2
\end{equation}

It follows that we can determine the value of $k$ by fitting the signal variances observed by collecting waveform samples at different intensities to Eq. \ref{eq:calibration2}. To do so we employ a 400 nm pulsed laser by modulating
its intensity through the use of different UV filters hosted in a remote-controlled filter wheel with transmittances (measured at $400$ nm) 1 (no filter), $0.83$, $0.71$, $0.53$, $0.28$ and $0.05$. The laser source is placed at $50$ cm from the PMT and aligned to the photocatode, to which the laser pulse travels through air. A pair of static filters (unchanged for different measurements) are placed between the wheel and the photocatode to bring the laser intensity down to the operational range. For each filter in the wheel we acquire $\sim$ 5000 waveforms. The procedure was repeated at photomultiplier supply voltage values of $1000$, $1200$, $1300$, $1500$ and $1600$ V. The fit of the data taken at a supply voltage of $1500$ V is shown in Fig. \ref{fig:fitPMTcalib}.

\begin{figure}
\centering
\includegraphics[width=0.7\textwidth]{img/1500Vcalib}
\caption{Fit of waveforms integral means acquired at $1500$ V to Eq. \ref{eq:calibration2}.}
\label{fig:fitPMTcalib}
\end{figure}
\input{./sections/Calibration/calpartab}

\paragraph{Calibrating the digitizer}

In order to estimate the phototube gain we need to determine what charge we observe from the anode after stimulation by an illumination of a given intensity. We know that if the signal measured by the ADC is $\mu$ when it collects $N$ anode charges, we can compute the PMT gain dividing $N$ by the number of photoelectrons expected at the cathode, $N_{pe}$, at the corresponding light intensity. $N_{pe}$ is readily determined from our knowledge of $k$, as in the previous paragraph.\\
We acquired rectangular waveforms with our NIM compatible waveform digitizer (CAEN N6472). Considering the digitizer input resistance $R = 50 \pm 0.5 \text{ }\Omega$, a pulse of amplitude $A$ [V] and duration $\tau$ will inject a total charge $Q = \tau A / R$ at the ADC input. We define the ratio between the intensity of a signal $\mu$ [ADU$\,\cdot $ s] and the expected charge integrated by the digitizer $Q$ as $c$, henceforth $Q = c\cdot\mu$. Dimensionally $c$ is equivalent to [$C\cdot$ ADU$^{-1}\, \cdot $ s$^{-1}$]. 
In order to estimate $c$ we acquired waveforms of different rectangular pulses %as in Tab. \ref{tab:digitizerCalibrationtab} 
and compared their mean integral intensity to the digitizer expected integrated charge.\\
The resulting estimate is $ c = (5.094\pm 0.007) \cdot 10^{-15} \,\,\, C\cdot $ADU$^{-1}\cdot $s$^{-1} $.

%\input{./sections/Calibration/digitcalibtable}

\paragraph{Gain-voltage curve}
The gain of a PMT changes according to the following law:
\begin{equation}
G(V) = (A V)^{b\cdot n}
\label{eq:gainvoltage}
\end{equation}
where $V$ is supply voltage, $n=10$ is the number of dynode stages and $b$ is a constant  determined by electrode structure and material \cite{hamamatsu_tubes}.
With $c$ and $k_V$ defined as in the previous paragraphs and indicating with $e$ the elementary charge, the gain at supply voltage $V$ is $G_V = c\cdot k_V/e$.
The voltage-gain curve is shown in Fig. \ref{fig:gaincurve}, along with the best fit to Eq. \ref{eq:gainvoltage}. Values of best fit parameters are  $A=6.80\pm0.2$ kV$^{-1}$ and $b= 0.5962\pm0.0088$. At an operational voltage of $1500$ V we estimate a gain value $G_{1500} = (1.04 \pm 0.04)\cdot 10^6$.


\begin{figure}[hb]
\centering
\includegraphics[width=0.7\textwidth]{img/gaincurve}
\caption{Gain-voltage curve and best fit to a power-law according to Eq. \ref{eq:gainvoltage}.}
\label{fig:gaincurve}
\end{figure}


==> sections/Calibration/calpartab.tex <==
\begin{table}[ht]
\centering
\resizebox{0.6\textwidth}{!}{%
\begin{tabular}{lP{4.0cm}P{4.0cm}}
\toprule
Gain [V] & k [ADU $\cdot$ s \ photoel.$^{-1}$] & $\sigma_k$ [ADU $\cdot$ s \ photoel.$^{-1}$] \\
\midrule
$1000$ &  $2.862$ & $ 0.081$ \\
$1200$ & $8.85$ & $0.29$ \\
$1300$ & $14.5$ & $1.2$ \\
$1500$ & $31.9$ & $3.3$ \\
$1600$ & $46.2$ & $2.6$ \\
\bottomrule
\end{tabular}}
\caption{Best values of $k$ parameters from fit to Eq. \ref{eq:calibration2}.}
\label{tab:calpartab}
\end{table}


==> sections/Calibration/digitcalibtable.tex <==
\begin{table}[]
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lll}
\toprule
A [mV] & T [ns] & Mean Integral [$ADC\cdot s$] \\
\midrule
$879 \pm 2$ & $66.47 \pm 0.04$ & $(1.88 \pm 0.02 ) \cdot 10^{-13}$ \\
$874 \pm 2$ & $100.69 \pm 0.12$ & $(3.42 \pm 0.03) \cdot 10^{-13}$\\
$872 \pm 2$ & $150.29 \pm 0.05$ & $(5.11 \pm 0.05) \cdot 10^{-13}$\\
$870 \pm 2$ & $200.15 \pm 0.03$ & $(6.81 \pm 0.07) \cdot 10^{-13}$\\
$879 \pm 2$ & $250.12 \pm 0.09$ & $(8.52 \pm 0.08) \cdot 10^{-13}$\\
$869 \pm 2$ & $300.07 \pm 0.05$ & $(1.02 \pm 0.01) \cdot 10^{-12}$\\
$871 \pm 2$ & $350.19 \pm 0.08$ & $(1.19 \pm 0.01) \cdot 10^{-12}$\\
\bottomrule
\end{tabular}}
\caption{Measured mean amplitude, durations and integral for different rectangular signals.}
\label{tab:digitizerCalibrationtab}
\end{table}


==> sections/RadTolerance/lyieldtable.tex <==
%\begin{table}[]
%\centering
%\resizebox{\textwidth}{!}{%
%\begin{tabular}{l|c|c|c|}
%\cline{2-4}
% & \multicolumn{1}{l|}{Peak Position [channels]} & \multicolumn{1}{l|}{Energy Resolution [\%]} & Received Dose [protons] \\ \hline
%\multicolumn{1}{|l|}{Before Irradiation} & $2324 \pm 19$ & $25.1 \pm 2.2$ & - \\ \hline
%\multicolumn{1}{|l|}{After Irradiation} & $2237 \pm 19$ & $27.6 \pm 2.3$ & $(2.95 + 0.05) \cdot 10^{10}$ \\ \hline
%\end{tabular}%
%}
%\caption{Peak positions and energy resolution before and after proton irradiation.}
%\label{tab:outputdegradation}
%\end{table}
\begin{table}[hb!]
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{llll}
\toprule
 &Peak Position [channels] & FWHM Energy Resolution [\%] & Dose [protons]  \\
\midrule
Before Irradiation & $2324 \pm 19$ & $25.1 \pm 2.2$ & - \\
After Irradiation & $2237 \pm 19$ & $27.6 \pm 2.2$ & $(2.95 + 0.05) \cdot 10^{10}$ \\
\bottomrule
\end{tabular}}
\caption{Peak positions and energy resolution before and after proton irradiation corresponding to an observed light-yield reduction of $3.7 \pm 1.2 \%$.}
\label{tab:outputdegradation_J1}
\end{table}


==> sections/RadTolerance/radtolerance.tex <==
\section{Light-Output degradation}
\label{sec:radtol}

\paragraph{Light-Output degradation} We observed a small degradation in light-output resulting from proton irradiation of GAGG:Ce up to a dose value roughly equivalent to the dose expected from $\gtrsim 10$ years of sun-synchronous orbit. Data for sample 'J2' are reported in Tab. \ref{tab:outputdegradation_J1} and Fig. \ref{fig:outputdegfig} implying a moderate light-yield reduction of $3.7 \pm 1.2 \%$, in agreement with the literature \cite{Yoneyama_2018}. 
Data come from integration of $\sim 5000$ GAGG:Ce acquisitions of scintillation events collected during beam 'dark mode',(cf. Sec. \ref{sec:expout}) irradiation with 70 MeV protons.
The beam being in low proton count regime allowed for operation of the PMTs at $800$ V without risking to burn them by the bright scintillation light. 
At this HV, photomultiplers had sufficient gain to be able to record single photon pulses and they were operated in coincidence. The single proton pulses recorded are shown in Fig. \ref{fig:outputdegfig}.\\

\begin{figure}[h!]
\centering
\includegraphics[width = 0.7\textwidth]{img/outputdegradation}
 	\caption{Maximum amplitude histogram from 70 MeV protons scintillation event, before (blue) and after (orange)  irradiation with $(2.95 + 0.05) \cdot 10^{10}$ protons. Only small variations in peak position were observed, accounting for reduction in light-yield of $3.7 \pm 1.2 \%$.}
	\label{fig:outputdegfig}
\end{figure}
\input{./sections/RadTolerance/lyieldtable}

